A Dataset and Baselines for Multilingual Reply Suggestion

Reply suggestion models help users process emails and chats faster. Previous work only studies English reply suggestion. Instead, we present MRS, a multilingual reply suggestion dataset with ten languages. MRS can be used to compare two families of models: 1) retrieval models that select the reply from a fixed set and 2) generation models that produce the reply from scratch. Therefore, MRS complements existing cross-lingual generalization benchmarks that focus on classification and sequence labeling tasks. We build a generation model and a retrieval model as baselines for MRS. The two models have different strengths in the monolingual setting, and they require different strategies to generalize across languages. MRS is publicly available at https://github.com/zhangmozhi/mrs.

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
\mz{Will move most of these contents somewhere else, and maybe remove this section.}

Automated reply suggestions is available in many applications including Gmail, Outlook, LinkedIn, Facebook Messenger, Micrsoft Teams, Uber, and etc.
SR task is in the domain of conversational AI, and can be compared to open domain dialog \cite{dialog citations} agents. However it is also quite different and perhaps closer to goal oriented dialog systems \cite{goal directed} to help users quickly finish a task (reply to a message), rather than engage in open chat which is the main objective in dialog systems.

Suggested replies have been modeled both as a generative process with sequence-to-sequence architectures \cite{kannan2016smart} commonly used in machine translation as well as a retrieval process \cite{henderson2017efficient, deb2019diversifying} which tended to be more popular in industrial settings due to better control over the suggestions. We compare the popular architectures in retrieval (matching architecture) and generation (s2s) in a multilingual setting. In addition, several conditional language generation models \cite{GPT2, GPT3, T5 etc} can be applied here which we leave for future work. 

As SR gets popular it becomes increasingly important to evaluate multiple languages for the task. Overall it is hard to imagine any NLP tasks without multi-lingual dataset support as a fairness and inclusion objectives in both research and production.

In \cite{conversation datasets} (Reddit, OpenSubtitles and Amazon Q/A) and \cite{Ubuntu dialog corpus} (ubuntu corpus) provides resources for generating data from publicly available repositories which maybe applicable for the SR task. However they are mostly in English, and multilingual dialog datasets are rare. In \cite{citation}, the ConvAI2 (Dinan et al., 2019a) dataset is extended to support six languages, using machine translations followed by followed by human refinement. This is a relatively small dataset and applicable for chat. Previous work has looked at dialog acts In  \cite{cite here} and task oriented dialog  /cite{task oriented} in multi-lingual in multilingual settings. Multilingual datasets also exist for standard NLP tasks such as Machine Translation, Language Understanding, Question-Answering to name a few, but to the best of our knowledge, the neither a dataset, nor any evaluations exists for the SR task.

Research has looked at both universal multi-lingual training as well as cross lingual transfer learning for extending models to multiple languages. More recently, fine-tuning pretrained multiligual text encoders for specific tasks has become an increasingly important technique for achieving multi-linguality. Multilingual extensions to popular pretrained models exist (MBERT etc, please cite). For generation models the laternatives include (unicoder, T5? etc). Several papers have improved their cross-lingual, multi-lingual, and zero-shot scenarios, by leveraging parallel data and different pre-training tasks \cite{devlin2018bert,conneau2019unsupervised,chi2020infoxlm}. We continue on such lines and evaluate the retrieval and generation approaches to SR using two standard encoders (MBERT, Unicoder). 
